Derivative-Based Koopman Operators for Real-Time Control of Robotic Systems

This paper presents a generalizable methodology for data-driven identification of nonlinear dynamics that bounds the model error in terms of the prediction horizon and the magnitude of the derivatives of the system states. Using higher-order derivatives of general nonlinear dynamics that need not be known, we construct a Koopman operator-based linear representation and utilize Taylor series accuracy analysis to derive an error bound. The resulting error formula is used to choose the order of derivatives in the basis functions and obtain a data-driven Koopman model using a closed-form expression that can be computed in real time. Using the inverted pendulum system, we illustrate the robustness of the error bounds given noisy measurements of unknown dynamics, where the derivatives are estimated numerically. When combined with control, the Koopman representation of the nonlinear system has marginally better performance than competing nonlinear modeling methods, such as SINDy and NARX. In addition, as a linear model, the Koopman approach lends itself readily to efficient control design tools, such as LQR, whereas the other modeling approaches require nonlinear control methods. The efficacy of the approach is further demonstrated with simulation and experimental results on the control of a tail-actuated robotic fish. Experimental results show that the proposed data-driven control approach outperforms a tuned PID (Proportional Integral Derivative) controller and that updating the data-driven model online significantly improves performance in the presence of unmodeled fluid disturbance. This paper is complemented with a video: https://youtu.be/9_wx0tdDta0.

==> TRO 2021 arXiv/packages.tex <==
\usepackage{cite}
\usepackage{url}
\usepackage{multicol}
\usepackage[normalem]{ulem}

\usepackage{titlesec}

\newcommand{\ssubsection}[1]{%
 \subsection*{\textbf{\raggedright\normalfont#1}}}

% For horizontal fraction
\def\nicefrac#1#2{\leavevmode%
 \raise.5ex\hbox{\small #1}%
 \kern-.1em/\kern-.15em%
 \lower.25ex\hbox{\small #2}}
 
\let\temp\rmdefault % add this before and after mathpazo package, to maintain same (more compact) font
\usepackage{mathpazo} % for plus minus symbol
\let\rmdefault\temp

\usepackage{tabularx,arydshln}

%% For pi in SI environment
\usepackage{siunitx}
\protected\def\numpi{\text{\ensuremath{\pi}}}
\sisetup{input-symbols = \numpi}

% \usepackage[bookmarks=true]{hyperref}
\usepackage[pdfauthor= { Giorgos Mamakoukas; Maria L. Castano; Xiaobo Tan; Todd D. Murphey},
 pdftitle={Derivative-Based Koopman Operators for Real-Time Control of Robotic Systems},
 pdfsubject={Derivative-Based Koopman Operators for Real-Time Control of Robotic Systems},
 pdfkeywords={Koopman Operators, Data-Driven Control, Error Bounds, Robotic Fish},colorlinks = true,
 % linkcolor = blue,
 urlcolor = blue,]{hyperref}

\usepackage{balance}
% \usepackage{flushend} % balanced columns of references at the end of document
\usepackage{siunitx} %% to fix distances between numbers and SI units
\sisetup{detect-all}
\sisetup{per-mode=symbol,inter-unit-product = \ensuremath{{}\cdot{}}}

\usepackage{adjustbox} % For table to shrink to fit column width

\usepackage{dcolumn}
\newcolumntype{L}{D{.}{.}{2,5}}

\usepackage{xcolor}
\usepackage{amsmath} 
\usepackage{amsfonts} % to use mathbb{R}
\usepackage{subcaption} % for subfigures
\usepackage{graphicx}
\usepackage{mwe}
\usepackage{tabularx} % fit table in column width

\usepackage{amsthm} % for bolded theorem
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}

\usepackage{amssymb}
\newlength{\tempdima}
\newcommand{\rowname}[1]% #1 = text % to add Text next to figures in Koopman/Backstepping
{\rotatebox{90}{\makebox[\tempdima][c]{\textbf{#1}}}}
\newcommand{\sgn}{\mathop{\mathrm{sgn}}} %% for sgn function
\usepackage{threeparttable} %% To add text centered below table 

\usepackage{soul}
\newcommand\hcancel[2][black]{\setbox0=\hbox{$#2$}%
\rlap{\raisebox{.3\ht0}{\textcolor{#1}{\rule{\wd0}{.5pt}}}}#2} 

\usepackage{tikz}
\usepackage{orcidlink}
